Deep Learning Based XIoT Malware Analysis: A Comprehensive Survey, Taxonomy, and Research Challenges

The Internet of Things (IoT) is one of the fastest-growing computing industries. By the end of 2027, more than 29 billion devices are expected to be connected. These smart devices can communicate with each other with and without human intervention. This rapid growth has led to the emergence of new types of malware. However, traditional malware detection methods, such as signature-based and heuristic-based techniques, are becoming increasingly ineffective against these new types of malware. Therefore, it has become indispensable to find practical solutions for detecting IoT malware. Machine Learning (ML) and Deep Learning (DL) approaches have proven effective in dealing with these new IoT malware variants, exhibiting high detection rates. In this paper, we bridge the gap in research between the IoT malware analysis and the wide adoption of deep learning in tackling the problems in this domain. As such, we provide a comprehensive review on deep learning based malware analysis across various categories of the IoT domain (i.e. Extended Internet of Things (XIoT)), including Industrial IoT (IIoT), Internet of Medical Things (IoMT), Internet of Vehicles (IoV), and Internet of Battlefield Things (IoBT).

==> tables/challenges_future_directions.tex <==
\begin{table}[h!]
\centering
\caption{Main Challenges and Future Research Directions.}
\label{tab:challenges_future_directions}
\rowcolors{2}{gray!25}{white}
\begin{tabular}{| m{2.5cm} | m{5cm} |}
\rowcolor{gray!25}
\hline
\textbf{Challenges} & \textbf{Future Research Directions} \\ \hline

\textbf{Security and Data Privacy Risks} &

Leveraging edge and fog computing for Real-Time Detection to enhance security and privacy by minimizing data transfer and processing locally

\\ \hline

\textbf{Resource Constraints in XIoT Devices} &

Optimizing Deep Learning models for resource-constrained XIoT devices using model Pruning, Quantization, and Federated Learning

\\ \hline

\textbf{Detection of Sophisticated and Evolving Malware Threats} &

Using continuous Learning frameworks to ensure that detection systems remain effective against new and evolving threats

\\ \hline

\textbf{Efficient Feature Extraction from Unstructured Data} &

1- Advanced NLP and Self-Supervised learning techniques can improve the accuracy and efficiency of feature extraction from unstructured data.

2-  XAI techniques can make the feature extraction process more transparent, helping to refine and improve these methods

\\ \hline

\textbf{Lack of Studies} &
 More comprehensive studies are needed to develop and benchmark new deep learning models tailored for XIoT environments
\\ \hline
\end{tabular}

\end{table}

